The Hamming Ball Sampler

We introduce the Hamming Ball Sampler, a novel Markov Chain Monte Carlo algorithm, for efficient inference in statistical models involving high-dimensional discrete state spaces. The sampling scheme uses an auxiliary variable construction that adaptively truncates the model space allowing iterative exploration of the full model space in polynomial time. The approach generalizes conventional Gibbs sampling schemes for discrete spaces and can be considered as a Big Data-enabled MCMC algorithm that provides an intuitive means for user-controlled balance between statistical efficiency and computational tractability. We illustrate the generic utility of our sampling algorithm through application to a range of statistical models.

==> extensions.tex <==
\section{Extensions of the Hamming Ball Sampler}

% \subsection{Further Technical Details about the Hamming Ball Sampler}



\subsection{Blocking strategies \label{sec:blockstrat}}


Here, we further discuss the use of Hamming Ball sampling, and its connection with Gibbs sampling, 
for the case $\bfX$ is just a large unstructured $D$-dimensional vector so that we iteratively apply conditional 
Hamming Ball moves to random blocks of $\bfX$. Notice that such algorithm was used in the simulated
sparse linear regression example and the real eQTL dataset.
   
At each iteration we divide the $\bfX$ variables into randomly chosen blocks $\bfx_i,\ i=1,\ldots,P$, so that they have common length $K = \text{length}(\bfx_i)$\footnote{If $D/P$ is not a integer, then the final block $\bfx_P$ will have size smaller than $K$. One way to deal with such case is to expand this block to make it have size $K$ by including some variables of the first block $\bfx_1$.}. However, instead of sampling each block conditional on the others 
using standard block Gibbs sampling (which will be infeasible when the block size is large), we use the Hamming Ball 
operation, i.e.\ $\bfu_i \leftarrow p(\bfu_i |\bfx_i)$ and $\bfx_i \leftarrow p(\bfx_i|\bfX_{-i}, \theta, \bfu_i, \bfy)$, 
and where the radius of the each Hamming Ball is $m$. 
%; see Section \ref{sec:staInfeqtL} for pseudo-code for the 
%whole algorithm. 
All different such schemes can be expressed by varying the 
block size $ K \in \{1,\dots,D\}$ and the radius $m \in \{1,\ldots,K\}$. Also these schemes can be visualized 
by a $D \times D$ upper triangular matrix where rows represent the radii and the columns the block sizes.
The diagonal elements of this matrix, where $m=K$, are precisely all standard block Gibbs Samplers, while the off-diagonal elements, where $m<K$, are block Hamming Ball schemes. 
%We shall refer to algorithms of this class as block Hamming Ball Samplers.    

The most effective block Hamming Ball scheme can correspond to a certain pair $(m,K)$ which   
shall trade off between computational time and sampling efficiency. The computational time is dominated by 
the number of operations needed to evaluate each conditional $p(\bfx_i|\bfX_{-i}, \theta, \bfu_i, \bfy)$ for $i=1,\ldots,P$. 
We can easily see that this involves $M \times P$ operations where $M$ is the volume of the individual 
Hamming Ball set ${\cal H}_m(\bfx_i)$ 
%\begin{equation}
%M = |{\cal H}_m(\bfx_i)| = \sum_{j=0}^m (S-1)^j {K \choose j},
%\label{eq:ballVolume}
%\end{equation}
and $P=D/K$ is the number of blocks. On the other hand, the sampling efficiency characterizes the sampler in terms of its  
ability to explore the probability distribution and jump between modes. Sampling efficiency 
depends also on the landscape and correlation structure of the probability distribution. For instance, if 
the posterior distribution $p(\bfX|\theta,\bfy)$ factorizes across all sites in $\bfX$ then any standard block Gibbs scheme 
with $m=K$, $m=1,\ldots,D$, will draw exact independent samples from the conditional posterior distribution over $\bfX$ and therefore it will have maximum 
sampling efficiency. However, the fastest scheme will be the one with $m=K=1$ since it will have the 
smallest computational time, and hence we can say that it has the maximum {\em overall efficiency}. For 
correlated posterior distributions the overall efficiency could be maximized by some pair $(m,K)$ that might not correspond to 
a standard block Gibbs Sampler. For instance,  Figure \ref{fig:efficiencyVerusCompexity} shows an example 
in variable selection in regression (generated exactly analogously as the example used in \emph{Results} section of the main paper and described further in Section \ref{sec:sparselinear}) where $\bfX$ is a binary vector of size $D=14$ and the posterior distribution 
has two completely symmetric modes so that jumping between modes requires simultaneously flipping the   
values of two specific variables. The right panel in Figure \ref{fig:efficiencyVerusCompexity} shows the overall efficiency, defined here as the
transition probability between the two modes over the time complexity, which is maximized for $(m,K)=(1,13)$.  


\begin{figure*}
\centering
\begin{tabular}{ccc}
{\includegraphics[scale=0.30]
{diagrams/fig_toyreg_complexity}} &
{\includegraphics[scale=0.30]
{diagrams/fig_toyreg1_efficiency}} & 
{\includegraphics[scale=0.30]
{diagrams/fig_toyreg1_efficiencyOverComplexity}} \\
Complexity  &  Sampling Efficiency & Overall Efficiency
%{\includegraphics[scale=0.23]
%{diagrams/fig_toyreg5_efficiencyOverComplexity}} 
\end{tabular} 
\caption{Sampling from a posterior distribution over $D=14$ binary variables having two symmetric modes so that jumping between the modes requires simultaneously flipping two certain binary variables. The left panel shows the 
computational complexity for all block Hamming Ball schemes. The middle panel shows the corresponding sampling efficiency which was defined as the transition probability between 
the two modes (an ideal exact sampler has maximum transition probability equal to $0.5$). Finally, the right panel displays the ratio between sampling efficiency and computational complexity
which is maximized for $(m,K)=(1,13)$. For all panels brighter colours indicate higher values.} 
\label{fig:efficiencyVerusCompexity}
\end{figure*}

\subsection{Randomness over the Hamming Ball radius \label{sec:randomm}}

A generalization of the algorithm is obtained by allowing block-wise random maximal Hamming distances.   
%Simple generalizations of the Hamming Ball Sampler allow a wide range of sampling schemes to be expressed that %incorporate standard Block Gibbs Samplers as special cases. 
More precisely, if we assume a varying radius for the individual Hamming Balls, then the conditional distribution over $\bfU$ is now uniform on the generalized Hamming Ball
$
{\cal H}_{\bfm}(\bfX) = \{ \bfU :  d( \bfu_i, \bfx_i ) \leq m_i, i=1, \ldots,P \},
$
where $\bfm = (m_1,\ldots,m_P)$ denotes the set of maximal distances for each subset of variables. Furthermore, we can allow $\bfm$, at each iteration, to be randomly drawn from a distribution $p(\bfm)$ which leads us to the following generalization of the algorithm:
\begin{align}
    (\bfU,\bfm) & \leftarrow p(\bfU|\bfX,\bfm) p(\bfm) \label{eq:u_hbsGener}, \\
	( \theta, \bfX ) & \leftarrow p(\theta, \bfX|\bfy, \bfU, \bfm), 
	\label{eq:thetaX_hbsGener}
\end{align}
where again the second step can be implemented either by applying two conditional Gibbs steps or a joint M-H step.
This scheme remains valid since  
essentially it is Gibbs sampling in an augmented probability model where we added the auxiliary variables $(U,\bfm)$. 
%In practical implementation, such a scheme can use a distribution $p(\bfm)$
%would place high prior probability on small values of individual $m$s where sampling iterations would be fast to %compute and enable efficient exploration of local structure but, with non-zero probabilities on larger values on %$m$, the sampler could still periodically consider larger portions of the model space that would allow more %significant changes to the configuration of $X$.

Furthermore, via the randomness over $\bfm$ we can again interpret standard block Gibbs Samplers as special cases.
When $p(\bfm)$ is such that at each iteration it randomly picks a single index $i$, sets $m_i= \text{length}(\bfx_i)$ and for the rest $j \neq i$ sets $m_j = 0$, the algorithm reduces to a block Gibbs Sampler. Since, in such a case, $\bfx_i$ would be freely sampled from its conditional $p(\bfx_i|\bfX_{-i},\theta,\bfy)$ while the remaining blocks $\bfX_{-i} = \{ \bfx_{j}: j \neq i \}$ would be frozen to their current values because the maximal distances of their individual Hamming Balls are zero. 

In practice using a varying or random $\bfm$ could lead to more efficient
variations of the Hamming Ball Sampler where, for instance, the vector $\bfm$ could be automatically tuned during
sampling to focus computational effort in regions of the sequence where there is most uncertainty in
the underlying latent structure of $\bfX$. The development of such variations of the main Hamming Ball 
algorithm is left for future work. 

\subsection{Non-uniform auxiliary Hamming Ball distributions \label{sec:nonuniform}}

As mentioned in the main paper the uniform distribution $p(\bfU|\bfX)$ over the auxiliary variables $\bfU$ 
defined inside the Hamming Ball ${\cal H}_m(\bfX)$ can more generally be modified to become an non-uniform one.  
For instance, a simple generalization is to assume an auxiliary distribution of 
the form 
\begin{equation}
p(\bfU|\bfX) = \frac{1}{Z_m} \exp( - \lambda d(\bfU,\bfX) ) \mathbb{I}(\bfU \in {\cal H}_m(\bfX)) 
= \frac{1}{Z_m} \prod_{i=1}^P \exp( - \lambda d(\bfu_i,\bfx_i) ) \mathbb{I}(\bfu_i \in {\cal H}_m(\bfx_i)),
\label{eq:PUXlambda} 
\end{equation}
where $d( \bfu_i, \bfx_i)$ denotes the Hamming distance as defined in the main text. Also, the parameter $\lambda \geq 0$ controls the variance of the distribution 
so that when $\lambda=0$, the above reduces to the uniform distribution while 
as $\lambda$ increases $p(\bfU|\bfX)$ places more and more probability mass 
towards the center $\bfX$ in a spherically symmetric way. Given that all vector $\bfx_i$s have size 
$K$ the overall normalizing constant can be written as $Z_m = M_{\lambda}^P$ where $M_{\lambda}$  
$$
M_{\lambda} = \sum_{j=0}^m e^{ - \lambda j } (S-1)^{j} { K \choose j },
$$
which is a weighted volume of each block-specific Hamming Ball that still remains independent from $\bfx_i$. Notice that in the above scheme $\lambda$ is an additional parameter that the user can tune in order to optimize sampling efficiency.  

In the most general  case the auxiliary distribution over $\bfU$ can have the form  
$$
p(\bfU|\bfX,\bfy) = \frac{1}{Z(\bfX)} f(\bfX, \bfU,\bfy) \mathbb{I}(\bfU \in {\cal H}_m(\bfX)) 
= \prod_{i=1}^P \frac{1}{Z(\bfx_i)} f(\bfx_i, \bfu_i,\bfy) \mathbb{I}(\bfu_i \in {\cal H}_m(\bfx_i)),
$$
where each $f(\bfx_i, \bfu_i,\bfy)$ is a function that takes non-negative values and each $Z(\bfx_i)$ 
is a normalizing constant that in general can depend on $\bfx_i$. For instance, notice that for the 
case in eq.\ (\ref{eq:PUXlambda}), $f(\bfx_i, \bfu_i,\bfy) = \exp( - \lambda d(\bfu_i,\bfx_i) )$.
The posterior conditional $p(\bfX|\bfU,\theta, \bfy)$  needed when sampling $\bfX$ can be written as 
$$
p(\bfX|\bfU,\theta, \bfy) \propto p(\bfy,\bfX,\theta) \frac{f(\bfX, \bfU,\bfy) \mathbb{I}(\bfU \in {\cal H}_m(\bfX))}{Z(\bfX)}.
$$
In our current simulations we experiment with the simplest (and perhaps the most practical) 
scheme where the auxiliary distribution is uniform and leave the above more elaborate cases for
the future.   


\subsection{Using Hamming Balls in a purely Metropolis-Hastings scheme \label{sec:MHscheme}}

An alternative way to use the restricted space defined by the Hamming Ball set 
${\cal H}_m (\bfX)$ is to construct directly a proposal distribution in a accept/reject 
Metropolis-Hastings (M-H) step in order to sample $\bfX$ without the use of the intermediate 
auxiliary variable $\bfU$. Specifically, if $\bfX^{(t)}$ is the value of the  current state 
we can define a proposal $Q(\bfX'|\bfX^{(t)})$ by slicing the exact model probability distribution  
around $\bfX^{(t)}$ according to
\begin{equation}
Q(\bfX'|\bfX^{(t)}) = 
\frac{ p(\bfy,\bfX', \theta) \mathbb{I}(\bfX' \in {\cal H}_m(\bfX^{(t)}) }
{Z_m(\bfX^{(t)})},
\end{equation}
where $Z_m(\bfX^{(t)}) = \sum_{\bfX' \in  {\cal H}_m(\bfX^{(t)}) }  p(\bfy,\bfX', \theta)$. 
Sampling then proceeds by proposing a certain $\bfX'$ from the above instrumental distribution
which is then accepted (i.e.\ the next state is set to  $\bfX^{(t+1)}=\bfX'$ ) with probability 
\begin{equation}
\min \left(1, \frac{p(\bfy,\bfX', \theta)}{p(\bfy,\bfX^{(t)}, \theta)}
\frac{ Q(\bfX^{(t)} | \bfX') }
{ Q(\bfX'|\bfX^{(t)}) }
 \right)  =  
 \min \left(1, \frac{p(\bfy,\bfX', \theta)}{p(\bfy,\bfX^{(t)}, \theta)}
\frac{ 
\frac{ p(\bfy,\bfX^{(t)}, \theta) \mathbb{I}(\bfX^{(t)} \in {\cal H}_m(\bfX') }
{Z_m(\bfX' )} 
}
{ \frac{ p(\bfy,\bfX', \theta) \mathbb{I}(\bfX' \in {\cal H}_m(\bfX^{(t)}) }
{Z_m(\bfX^{(t)})} 
} \right) = 
 \min \left(1, \frac{Z_m(\bfX^{(t)})}{Z_m(\bfX')} 
 \right),
\end{equation} 
while otherwise $\bfX'$ is rejected and $\bfX^{(t+1)} = \bfX^{(t)}$. Notice that 
$Z_m(\bfX^{(t)})$ is the probability mass or volume of the sliced part of the model 
around $\bfX^{(t)}$ which is the state we are starting from, while similarly
$Z_m(\bfX')$ is the volume around the state we attempt to move into. 
Thus, in order to satisfy detailed balance the above M-H probability essentially reduces to 
the ratio between the probability volume around the current state and the volume around 
the proposed state.  

While the above scheme is a valid MCMC mechanism has certain limitations when compared to 
the auxiliary variable construction used in the Hamming Ball Sampler. More precisely, controlling the acceptance 
rate in the above scheme, when sampling $\bfX$, is difficult and sampling might exhibit unpredictably 
low acceptance rate so that the chain can get stuck to the same state for many iterations. If the user wishes 
to increase the acceptance rate then he must increase the radius $m$ of the Hamming Ball so that 
when $m$ takes its maximum value, i.e.\ equal to the block size $K$, then $Z_m(\bfX^{(t)}) = 
Z_m(\bfX') = p(\bfy,\theta)$ and sampling reduces to an exact Gibbs step where we simulate
from the exact posterior conditional $p(\bfX|\theta,\bfy)$. 
Of course, such a scheme is computationally not feasible in general. A second limitation 
is that the amount of exploration based on the above mechanism is half the amount of exploration of the Hamming Ball Sampler
that uses the auxiliary variable $\bfU$. This is because now the next state $\bfX^{(t+1)}$ can differ from the current $\bfX^{(t)}$ in at most $m P$ elements. In contrast, the Hamming Ball 
Sampler while it has the same computational cost with the above pure M-H algorithm, at the same time 
through the sampling of the auxiliary variables $\bfU$ allows to always 
accept any proposed $\bfX^{(t+1)}$ and on top of that the amount of 
exploration is doubled by allowing $\bfX^{(t+1)}$ to differ from $\bfX^{(t)}$ at maximum in 
$2 m P$ elements.  

Finally, notice that schemes similar to the above M-H approach haver been used before for 
variable selection applications and particularly in the Metropolized Shotgun Stochastic Search algorithm 
(see section 4.1 in \cite{shotgun2007}). 


